Online nonparametric regression with Sobolev kernels

In this work we investigate the variation of the online kernelized ridge regression algorithm in the setting of $d-$dimensional adversarial nonparametric regression. We derive the regret upper bounds on the classes of Sobolev spaces $W_{p}^{\beta}(\mathcal{X})$, $p\geq 2, \beta>\frac{d}{p}$. The upper bounds are supported by the minimax regret analysis, which reveals that in the cases $\beta> \frac{d}{2}$ or $p=\infty$ these rates are (essentially) optimal. Finally, we compare the performance of the kernelized ridge regression forecaster to the known non-parametric forecasters in terms of the regret rates and their computational complexity as well as to the excess risk rates in the setting of statistical (i.i.d.) nonparametric regression.

==> macromine01.tex <==
%Packages standard

% Fonts

\newcommand{\mtc}{\mathcal}
\newcommand{\mbf}{\mathbf}

% Some black magic to remove annoying extra spaces before/after \left* and \right*

\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}


% Accents tildes over/underline etc

\newcommand{\wt}[1]{{\widetilde{#1}}}
\newcommand{\wh}[1]{{\widehat{#1}}}
\newcommand{\ol}[1]{\overline{#1}}
%\newcommand{\ul}[1]{\underline{#1}}

% different delimiters 

\RequirePackage{xstring}

\newcommand{\ind}[1]{{\mbf{1}\{#1\}}}
\newcommand{\paren}[2][a]{%
\IfEqCase{#1}{%
{a}{\left(#2\right)}%
{0}{(#2)}%
{1}{\big(#2\big)}%
{2}{\Big(#2\Big)}%
{3}{\bigg(#2\bigg)}%
{4}{\Bigg(#2\Bigg)}%
}[\PackageError{paren}{Undefined option to paren: #1}{}]%
}
\newcommand{\norm}[2][a]{%
\IfEqCase{#1}{%
{a}{\left\lVert#2\right\rVert}%
{0}{\lVert#2\rVert}%
{1}{\big\lVert#2\big\rVert}%
{2}{\Big\lVert#2\Big\rVert}%
{3}{\bigg\lVert#2\bigg\rVert}%
{4}{\Bigg\lVert#2\Bigg\rVert}%
}[\PackageError{norm}{Undefined option to norm: #1}{}]%
}
\newcommand{\brac}[2][a]{%
\IfEqCase{#1}{%
{a}{\left[#2\right]}%
{0}{[#2]}%
{1}{\big[#2\big]}%
{2}{\Big[#2\Big]}%
{3}{\bigg[#2\bigg]}%
{4}{\Bigg[#2\Bigg]}%
}[\PackageError{brac}{Undefined option to brac: #1}{}]%
}
\newcommand{\inner}[2][a]{%
\IfEqCase{#1}{%
{a}{\left\langle#2\right\rangle}%
{0}{\langle#2\rangle}%
{1}{\big\langle#2\big\rangle}%
{2}{\Big\langle#2\Big\rangle}%
{3}{\bigg\langle#2\bigg\rangle}%
{4}{\Bigg\langle#2\Bigg\rangle}%
}[\PackageError{inner}{Undefined option to inner: #1}{}]%
}

\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}

% Misc

\newcommand{\np}{_{_-}}
\newcommand{\pp}{_{_+}}
\newcommand{\bydef}{\coloneqq}       % an alternative to defeq
%\newcommand{\defeq}{\stackrel{\cdot}{=}} % this is for
                                % definition-equal, not for number 2
                                % [This comment is (c) Gabór L. ]
\renewcommand{\star}{*}
% Probabilistic operators

\newcommand{\var}[2][a]{{\rm Var}\brac[#1]{#2}}
\newcommand{\cov}[2][a]{{\rm Cov}\brac[#1]{#2}} 
\newcommand{\e}[2][a]{\mbe\brac[#1]{#2}}
\newcommand{\ee}[3][a]{\mbe_{#2}\brac[#1]{#3}}
\newcommand{\prob}[2][a]{\mbp\brac[#1]{#2}}
\newcommand{\probb}[3][a]{\mbp_{#2}\brac[#1]{#3}}
\DeclareMathOperator{\fatt}{fat}


% Operators

\def\argmin{\mathop{\rm Arg\,Min}\limits}
\def\argmax{\mathop{\rm Arg\,Max}\limits}
\def\sgn{\mathop{\rm Sgn}\limits}
\def\tr{\mathop{\rm Tr}\limits}
\DeclareMathOperator{\rank}{rank}

% letters 

\newcommand{\al}{\alpha}
\newcommand{\om}{\omega}
\newcommand{\eps}{\varepsilon}
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\la}{\lambda}

% letters diff
\def\cA{{\mtc{A}}}
\def\cB{{\mtc{B}}}
\def\cC{{\mtc{C}}}
\def\cD{{\mtc{D}}}
\def\cE{{\mtc{E}}}
\def\cF{{\mtc{F}}}
\def\cG{{\mtc{G}}}
\def\cH{{\mtc{H}}}
\def\cI{{\mtc{I}}}
\def\cK{{\mtc{K}}}
\def\cL{{\mtc{L}}}
\def\cM{{\mtc{M}}}
\def\cN{{\mtc{N}}}
\def\cO{{\mtc{O}}}
\def\cP{{\mtc{P}}}
\def\cQ{{\mtc{Q}}}
\def\cR{{\mtc{R}}}
\def\cS{{\mtc{S}}}
\def\cT{{\mtc{T}}}
\def\cU{{\mtc{U}}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

% letters bold 
%\def\bx{\bf{x}}



% abbrev letters mathbb

\newcommand{\mbe}{\mathbb{E}}
\newcommand{\mbr}{\mathbb{R}}
\newcommand{\mbp}{\mathbb{P}}
\newcommand{\mbq}{\mathbb{Q}}
\newcommand{\mbi}{\mathbb{I}}
\newcommand{\mbn}{\mathbb{N}}
\newcommand{\mbz}{\mathbb{Z}}
\newcommand{\mbs}{\mathbb{S}}


% abbrev bold letters

\newcommand{\bA}{{\mbf{A}}}
\newcommand{\bD}{{\mbf{D}}}
\newcommand{\bG}{{\mbf{G}}}
\newcommand{\bI}{{\mbf{I}}}
\newcommand{\bW}{{\mbf{W}}}
\newcommand{\bX}{{\mbf{X}}}
\newcommand{\bY}{{\mbf{Y}}}
\newcommand{\bZ}{{\mbf{Z}}}


\newcommand{\bp}{{\mbf{p}}}
\newcommand{\bs}{{\mbf{s}}}
\newcommand{\bx}{{\mbf{x}}}
\newcommand{\by}{{\mbf{y}}}
\newcommand{\bz}{{\mbf{z}}}
\newcommand{\bw}{{\mbf{w}}}
\newcommand{\bv}{{\mbf{v}}}

% frak
\newcommand{\fR}{{\mathfrak{R}}}
\newcommand{\fP}{{\mathfrak{P}}}
\newcommand{\fK}{{\mathfrak{K}}}
\renewcommand{\hat}{\widehat}



%
% \newcommand{\red}[1]{\textcolor{red}{#1}}


% definition of not in a set
%\Umathchardef\xnot="3 \symoperators "0338
%\AtBeginDocument{\renewcommand\not[1]{#1\xnot}
%\renewcommand{\notin}{\in\xnot}}


% TODO command

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% A command to put notes in a draft

\newcounter{nbdrafts}
\setcounter{nbdrafts}{0}
\makeatletter
\newcommand{\checknbdrafts}{
\ifnum \thenbdrafts > 0
\@latex@warning@no@line{**********************************************************************}
\@latex@warning@no@line{* The document contains \thenbdrafts \space draft note(s)}
\@latex@warning@no@line{**********************************************************************}
\fi}
%\newcommand{\todo}[1]{\addtocounter{nbdrafts}{1}{\color{red} #1}}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

